Rewrite to Reinforce: Rewriting the Binary to Apply Countermeasures against Fault Injection

Fault injection attacks can cause errors in software for malicious purposes. Oftentimes, vulnerable points of a program are detected after its development. It is therefore critical for the user of the program to be able to apply last-minute security assurance to the executable file without having access to the source code. In this work, we explore two methodologies based on binary rewriting that aid in injecting countermeasures in the binary file. The first approach injects countermeasures by reassembling the disassembly whereas the second approach leverages a full translation to a high-level IR and lowering that back to the target architecture.

==> sections/3.0-lifting.tex <==
% \subsection{Rewriting the Binary} 
% \label{sec:rewriting}
% In this section, we will go though the publicly available binary rewriting solutions and compare their approach with regard to structural recovery, data type extraction, and limitations on supported architectures. 

% \begin{figure}[!]
%     \centering
%     \includegraphics[width=\linewidth]{./img/pipeline.pdf}
%     \caption{Coverage percentage achieved over for the cover sizes of different sizes\label{fig:pipeline}}
% \end{figure}

% \subsection{Definition} \label{sec:definiion} Binary rewriting denoted as the process of modifying a compiled program such a way it remains executable and functional without having access to the source-code. There are two types of binary modifiers, static and dynamic. In static approach, results of the modification will be saved as a copy for future execution on a persistent memory like disk. However, dynamic rewriting is applied during the program execution. In this paper we are focusing on static binary rewriting technique and compare the tools following this scheme.
Binary rewriting is the process of translating the binary file into a new IR, modifying the IR, and compiling it back to binary in a way that it remains functional without having access to the source-code.  
There are two types of binary modifiers, static and dynamic. In the static approach, results of the modification will be saved as a copy for future execution on a persistent memory like disk. However, dynamic rewriting is applied during the program execution. 
In this paper, we focus on the static binary rewriting technique.
% Based on Figure \ref{fig:pipeline}, from a high-level view, in the first step (\circled{1}), a binary rewriter receives a file in a binary stream format as input and passes it to the disassembler for decoding the instructions, and retrieving global variables and sections. Decoded instructions help the step \circled{2} in building the control and data flow, recovering data types, and function boundaries to semantically enriching the context with metadata lost during the compilation.

% Transformation step (\circled{3}) is about modifying the target binary in a way that mutated output is a working executable. In this research we focus more on the platforms that help us in statically rewriting the binary and we exclude dynamic binary rewriting which is called Dynamic Binary Instrumentation (DBI). 

% \subsection{Static Binary Rewriting}
There are three known static rewriting schemes. The oldest one is based on \textit{detouring} at assembly level. \textit{Detouring} works by hooking out the underlying instruction. 
% There are two flavours of detouring technique, \textit{patch-based instrumentation} and \textit{replica-based instrumentation}. \textit{Patch-based instrumentation} replaces the instruction with an unconditional branch into a new section contains instrumentation, replaced instruction, and a control flow transfer back to the patch point. Detouring is a direct rewriting and is ISA dependant which makes the approach inconvenient. This approach introduces a high performance degradation given the two control transfers at patch points. 
% \textit{Replica-based instrumentation} method places jump instructions at control flow changing destinations to a replicated code section containing both a copy of the original code and instrumentation. All memory references in this section are modified to maintain less control flow transfers between original and replicated section. While the performance of this approach is better compared to the \textit{patch-based}, the size of the resulting binary is noticeably increased. 
The detouring approach is known to introduce high performance degradation and extra code size overhead.

% % describe reassembling the disassembly
% \textit{Reassembleable disassembly} works by recovering relocatable assembly code which instrumentation could be inlined and reassembled back to a working binary. This approach first introduced by UROBOROS \cite{wang2016uroboros} and then expanded by improving on top of the idea in Ramblr \cite{wang2017ramblr}. This approach enhances the performance since inlined assembly avoids inserting control flow changing instructions at instrumentation points. As a result, performance penalty causing by jump instructions alleviated in this technique. 
\textit{Reassembleable disassembly} is another static rewriting scheme which works by recovering relocatable assembly code in which the instrumentation could be inlined and reassembled back to a working binary. This approach was first introduced by UROBOROS \cite{wang2016uroboros} and later was expanded and improved in Ramblr \cite{wang2017ramblr}. Compared to \textit{detouring}, this approach has a lower performance penalty as it implements changes locally.
% enhances the performance since inlined assembly avoids inserting control flow changing instructions at instrumentation points. As a result, the performance penalty caused by jump instructions is alleviated in this technique. 
% In our first countermeasure insertion technique, we use GrammaTech's \textit{Ddisasm} tool \cite{251538} which is a binary rewriter of this type.

% \textit{Full-translation} approach works upon translating a low-level machine code to a high-level intermediate representation (IR) using a compiler-based front-end for architecture independent binary rewriting. This process called \textit{lifting} the binary and assembling the IR back to a working executable denoted as lowering. Advantages of lifting the binary to a high-level IR are two folds. First, relying on IR makes the rewriting framework ISA-agnostic, hence supports more architectures. Second, providing the ability to apply program analysis techniques like Value Set Analysis (VSA) \cite{balakrishnan2004analyzing} and optimization passes like Simple Expression Tracker (SET) and Offset Shifted Register Analysis (OSRA) conveniently \cite{di2017rev}. 
\textit{Full-translation} is the last static rewriting scheme. This scheme translates a low-level machine code to a high-level intermediate representation (IR) using a compiler-based front-end for architecture independent binary rewriting. 
The advantage of lifting the binary to a high-level IR is two fold. First, relying on IR makes the rewriting framework ISA-agnostic, hence supports more architectures. Second, working on a high-level IR provides the opportunity to apply program analysis techniques like Value Set Analysis (VSA) \cite{balakrishnan2004analyzing} and optimization passes like Simple Expression Tracker (SET) and Offset Shifted Register Analysis (OSRA) conveniently \cite{di2017rev}. 
% In our second countermeasure insertion method, we use Revng's \textit{revng} tool \cite{di2017rev} that lifts the binary file to LLVM-IR and enables applying changes to the program in a high level of abstraction. 

% % a comparison between different binary rewriting techniques. 1. retrowrite 2. ramblr 3. datalog disassembly 4. UROBOROS 5. rev.ng 6. binrec
% % comparison metrics: 1. architecture support 2. rely on availability of symbols 3. size of the resulting binary 4. control flow recovery? 5. data type recovery? 6. intermediate-representation? 7. availability 8. SSA? 9. symbolic labels? 

% \subsection{Comparison of Binary Rewriters}



==> sections/long/countermeasures.tex <==
% \section{Experimental Results} \label{sec:experiments}
% \todo[inline, color=green!40]{
% Experimental results and comparison of them with results of other works 
% }
\subsection{Local Protections}
% In this section, we describe the redundant computation-based countermeasures that we used in our case studies for our faulter+rewriter approach. 

In the faulter+rewriter approach, we are able to insert protected code patterns locally. The following is the description of these redundant computation-based protections.

\subsubsection{Protecting {\tt mov} Instruction} To protect the {\tt mov} operation against fault attacks, there are two protection patterns that can be applied locally (Table~\ref{tab:mov}). In the first protected code, the {\tt mov} instruction is simply duplicated so that in case the first one is skipped by an injected fault, the second one will be executed.
In the second protected code, after executing the {\tt mov} operation, the result of the two memory locations are compared and in case of an inconsistency, a faulthandler is called.
\input{tables/mov}

\subsubsection{Protecting the {\tt cmp} Instruction}
We can protect a {\tt cmp} instruction against fault attacks in two ways (Table~\ref{tab:cmp}). Either by simply duplicating the instruction so that if one of them is skipped, the other copy will do the comparison. However, to be able to detect and recover from faults, we need to take a longer approach in which we execute the comparison twice and compare their resulting flags. To this end, we use the {\tt pushfq} instruction in x86-64 ISA which requires a valid stack pointer ({\tt rsp}). Due to Intel's red zone, we have to subtract 128 bytes from {\tt rsp} to jump out of the red zone.
\input{tables/cmp}

\subsubsection{Protecting the {\tt j<cond>} operation}
By hardening the conditional jump operations, we fix glitches that change the jump condition. In the protected code shown in Table~\ref{tab:jmp}, we use the flags register and match this to the expected flag in the jump-target and the fallthrough of a branch.
\input{tables/jmp}

% \subsection{Conditional Branch Hardening} 
\subsection{Holistic Protection} 
\label{sec:countermeasure}
% In this case study, we describe a novel countermeasure which is not easy to implement directly on the executable binary file but can be implemented easily using the proposed hybrid approach in Section~\ref{sec:hybrid}. Similarly, the same countermeasure can be applied to a software implementation when the source code is available at compile-time.


In this section, we provide the description of a conditional branch hardening method that we later use in our case studies for the hybrid countermeasure implementation approach.

% \subsubsection{Motivation}
% The majority of the existing countermeasures against fault attacks focus on data faults. However, fault attacks targeting only the control flow of a program can have significant results while dodging such data-oriented countermeasures. On the other hand, Control Flow Integrity (CFI) has been extensively studied in previous works. In such scenarios, the goal is to ensure any program flow taken at run-time is legitimate, \textit{i.e.} one of the possible paths in the Control Flow Graph (CFG) of the program. To prevent fault attacks, this type of CFI is necessary but not sufficient. For instance, 
% CFI solutions like Opaque Control-Flow Integrity \cite{mohan2015opaque} will protect against some code-reuse attacks such as Return-Oriented Programming (ROP) \cite{shacham2007geometry}, however, 
% if a fault attack affects the program in such a way that the flow would still fit into the set of legitimate possible paths but the program would bypass some security checks, the attack would effectively go unnoticed to the CFI solutions.

% One of the scenarios where this can happen is a conditional branch. For example, imagine a simple program that receives a pin code and only if the pin code is correct, resumes the program to execute some functions. In the assembly code (equally the machine code and the executable file) of this program, there will be a comparison instruction to compare the inserted pin code and its expected correct value, as well as a conditional branch instruction that, based on the result of the comparison, goes to a successor basic block. The following shows the assembly code and Figure~\ref{fig:branchInst} shows the CFG of this branch operation. 
Imagine a simple program that receives a pin code and only if the pin code is correct, resumes the program to execute some functions. In the assembly code (equally the machine code and the executable file) of this program, there will be a comparison instruction to compare the inserted pin code and its expected correct value, as well as a conditional branch instruction that, based on the result of the comparison, goes to a successor basic block. The following shows the assembly code and Figure~\ref{fig:branchInst} shows the CFG of this branch operation. 


\begin{verbatim}
        cmp rs1, rs2
        bne target2
        ...
    target1:
        ...
    target2: 
        ...
\end{verbatim}
In the case of Control Flow Integrity (CFI), going from BB1 to either of BB2 or BB3 does not raise any issues since they both are valid paths in the CFG. However, if an injected fault results in taking the wrong branch, it will be an unnoticed fault.  

\begin{figure}[htb]
    \centering
    \includegraphics[width=.4\linewidth]{figures/experiment/conditionalBranchCFG.pdf}
    \caption{CFG of a simple branch instruction}
    \label{fig:branchInst}
\end{figure}

\begin{figure}[tb]
    \centering
    \includegraphics[width=.8\linewidth]{figures/experiment/countermeasureCFG.pdf}
    \caption{CFG of the example conditional branch hardening}
    \label{fig:countermeasure_cfg}
\end{figure}

% \begin{figure*}
%  \centering
%  \subfigure[Simple branch instruction]{\includegraphics[width=.3\linewidth]{figures/experiment/conditionalBranchCFG.pdf}}\quad
%   \subfigure[CFG of the countermeasure with example settings]{\includegraphics[width=.5\linewidth]{figures/experiment/countermeasureCFG.pdf}}
% \end{figure*}

There are three fault targets that can result in the incorrect branch being taken. The first is when the input data to the comparison (namely {\tt rs1} and/or {\tt rs2}) are faulted such that the comparison result gets subverted. The second is when the comparison flag is affected by the fault. And the last is when the instruction is changed such that the incorrect branch is taken. One of the possible causes of changes on the instruction is when the branch instruction ({\tt bne} in our example code) is skipped which means the fall-through code ({\tt target1}) will be executed regardless of the compare result. Another possible attack is a bitflip that affects the predicate of the comparison. For instance, in both ARM and RISC-V ISAs the {\tt bne} and {\tt beq} are only different in one bit of their opcodes while having the opposite functionalities.


% Schilling et al. \cite{8342268} propose a countermeasure that can protect against mistaken branches, however, their countermeasure assumes that data and all performed operations on it are encoded redundantly which implies a high overhead. In another work, Werner et al. \cite{werner2018sponge} propose the sponge-based methodology in which every instruction will be encrypted at compile time with an authenticated encryption algorithm and decrypted and authenticated at run-time. However, this requires modification in the hardware processor to decrypt each instruction and given the long turn-out of processor design and tape-out, in many scenarios this is not achievable. 

% \subsubsection{Definition}

We propose a countermeasure for the mentioned conditional branch vulnerability that would not require any modification neither to the processor hardware nor to the other parts of the program, and hence, can be easily combined with other countermeasures.
In this approach, we assign a unique ID to each basic block ($UID_{BB}$) at compile time. We then choose an algorithm in the form of \(h(UID_{src},UID_{dst},cmp\_res)\) in which $UID_{src}$ and $UID_{dst}$ represent the $UID$ assigned to the source and destination basic blocks of the branch instruction respectively and $cmp\_res$ represents the result of the compare instruction. The dependency of the $h$ algorithm on the $UID$s makes its value unique for different branch instructions in the CFG while its dependency on the $cmp\_res$ makes it unique to different edges from the same branch instruction. The simplicity level of the $h$ function can be decided based on the required security properties of the program (an example for this algorithm is given in Algorithm \ref{alg:h_alg}). The $h$ algorithm will calculate a checksum at run-time based on the fixed $UID$s assigned at compile-time and the dynamically-evaluated compare result. The calculated checksum will be stored in a register and checked in the destination basic blocks. At the destination blocks, since the expected $cmp\_res$ for the taken edge is known, the expected value of $h$ is known. Therefore checking the evaluated value only requires reading the register value and comparing it with the expected value. When the register does not contain the expected value, we jump to a fault-response basic block.




% \subsubsection{Implementation}
% TODO Definition of $h$ and the fault-response function.

As an example of this method, we chose a simple option for the $h$ algorithm and implemented it as an optimization pass in the LLVM tool-chain. In this example, the checksum is calculated as the XOR result of the UID of the taken destination block and that of the source block ($UID_{dst} \oplus UID_{src}$).
The pseudo-code of the calculation procedure of this checksum in LLVM is shown in Algorithm~\ref{alg:h_alg} where $cmp\_res$ is the result of the comparison for the conditional branch, and $UID_{Tdst}$, $UID_{Fdst}$, and $UID_{src}$ are the UIDs assigned to the true destination (the destination taken when the comparison result is true), the false destination (the destination taken when the comparison result is false), and the source block respectively. The $mask$ shown on line 4 will have the value of all ones if the comparison result is false and the value of all zeros if the comparison result is true. The checksum will be located in one register and each of the destination blocks will evaluate whether the value of the checksum is correct. 

Furthermore, we made this evaluation duplicated; 
Figure~\ref{fig:countermeasure_cfg} shows the CFG of this implementation protecting the conditional branch shown in Figure~\ref{fig:branchInst}. We run the comparison instruction once ({\tt C\textsubscript{1}}), and calculate the checksum based on its result and keep it in a register ({\tt D\textsubscript{1}}). We perform this calculation another duplicated time and keep the result in a new register ({\tt D\textsubscript{2}}). We then perform the comparison again and run the branch based on the result of the second comparison ({\tt C\textsubscript{2}}). As shown by the orange boxes, the expected value of the checksum is different for the out-going edges of the source block ({\tt N\textsubscript{1}} vs. {\tt N\textsubscript{2}}). 
In the destination blocks, we check both copies of the checksum stored in registers against the expected values in a nested fashion. The green blocks show the nested checksum validations and the blue blocks represent the fault-response. As a simple example, the fault-response can be aborting the execution (in the {\tt flt\_respx} basic blocks).


 \begin{algorithm}[H]
%   \algsetup{linenosize=\tiny}
     \small
 \caption{Simple example algorithm for $h$}
 \label{alg:h_alg}
 \begin{algorithmic}[1]
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
 \REQUIRE $cmp\_res$, $UID_{Tdst}$, $UID_{Fdst}$, $UID_{src}$
 \ENSURE $checksum$
 \\ \textit{Generate unique checksums for edges} :
 \STATE $const_{Tdst} \gets UID_{Tdst} \oplus UID_{src}$
 \\ \STATE $const_{Fdst} \gets UID_{Fdst} \oplus UID_{src}$
 \\ \textit{Calculate checksum of the branch} :
  \STATE $cmp\_ext \gets zero\_extend(cmp\_res)$
  \\ \STATE $mask \gets cmp\_ext - 1$
  \\ \STATE $checksum \gets (\neg mask \land const_{Tdst}) \lor (mask \land const_{Fdst})$
%  \\ \textit{LOOP Process}
%   \FOR {$i = l-2$ to $0$}
%   \STATE statements..
%   \IF {($i \ne 0$)}
%   \STATE statement..
%   \ENDIF
%   \ENDFOR
%  \RETURN $P$
 \end{algorithmic}
 \end{algorithm}

As mentioned in the previous part, the goal of the proposed countermeasure is to prevent an attacker from causing a conditional branch to take the incorrect branch by injecting faults. In this scenario, if the attacker tries to skip one of the comparison instructions or change it to compute the inverse output, the checksum validation process will be able to catch the injected error. If the adversary intends to bypass this process, they would need to inject the exact same fault in both comparison results. In Section~\ref{sec:casestudies}, we show a simulated analysis of the effectiveness of this countermeasure.

The overall overhead of this countermeasure depends on the number of conditional branches that we want to protect and therefore is highly application-specific. Table~\ref{tab:qualOverhead} shows how many instructions are required to replace a simple conditional branch by this method. We implement the conditional branch hardening as an optimization pass in the LLVM compiler tool-chain. Therefore, its translation will differ for different target architectures based on how the instruction-lowering is done for that architecture in the LLVM back-end. 
% In the following we provide a qualitative analysis of the overhead resulted from this countermeasure.

\input{tables/qualitative_analysis_overhead}


% \paragraph{Transforming to IR} We first transform the binary file to an IR. This transformation is called binary lifting. In Section~\ref{sec:binarylifter}, we describe a few existing binary lifters and compare their efficacy for our goal. The IR should make the countermeasure implementation easier and automatic. In this work, we choose LLVM-IR because many open-source tools are already available to work on this IR and also many open-source binary-lifters exist to lift binaries to LLVM-IR. We start from lifting the binary executable file of a program to the LLVM-IR using the {\tt revng} tool \cite{di2017rev} which is a binary analysis framework based on QEMU and LLVM. The resulting IR, contains all the hierarchy levels in an LLVM-IR, \textit{i.e.} starting from the higher-level, module, function, basic block, and instruction. 

% \paragraph{Implementing the countermeasure} Once the IR is available, we automate the countermeasure implementation on the chosen IR. In our approach, this implementation will be a part of LLVM tool-chain. Depending on the requirements of the countermeasure, it will be added as an optimization pass to the middle-end of LLVM structure or as a target-specific pass to the back-end of LLVM. In our conditional branch protection scheme, we only need an optimization pass in the middle-end of LLVM. 
% % To protect the conditional branches, our focus is mainly on the basic blocks of a program. 
% First, we need to find the conditional branches. The basic block hierarchy level in LLVM-IR is quite useful for this purpose. A basic block is a set of instructions that run consecutively. Therefore, if any type of branch operation exists in a program, it will be the last instruction, \textit{i.e.} the terminator, of a basic block. Hence, by checking the terminator of each basic block we can find the conditional branches.
% The conditional branch instruction in LLVM-IR gives us access to the condition flag register. By knowing the register in which the condition flags are stored, we can add a logic that dynamically calculates the checksum value based on the condition flags. 

% \paragraph{Compiling back to binary} Once the countermeasure is implemented in IR, we compile the IR back to an executable binary. In our approach, LLVM's {\tt llc} tool is used for this purpose. Depending on the countermeasure, extra steps, in the form of LLVM back-end passes, might be necessary to make sure the compiler does not omit the implemented countermeasure.

==> sections/long/jmp_table.tex <==
\begin{table}[]
\caption{Local protection for conditional jump operation}
\centering
\scalebox{0.8}{

\begin{tabular}{ll}
\hline
\multicolumn{1}{c}{\textbf{original}}                                                                                & \multicolumn{1}{c}{\textbf{protected}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ \hline
\begin{tabular}[c]{@{}l@{}}j\textless{}cond\textgreater jumptarget\\ fallthrough: ...\\ jumptarget: ...\end{tabular} & \begin{tabular}[c]{@{}l@{}}j\textless{}cond\textgreater newjumptarget\\ lea rsp, {[}rsp-128{]}\\ push rcx\\ pushfq\\ set cl\\ cmp cl, 0\\ je newfallthroughjmp\\ call faulthandler\\ newfallthroughjmp:\\ popfq\\ pop rcx\\ j\textless{}cond\textgreater fallthrough\\ call faulthandler\\ newjumptarget:\\ lea rsp, {[}rsp-128{]}\\ push rcx\\ pushfq\\ set cl\\ cmp cl, 1\\ je newjumptargetjmp\\ call faulthandler\\ newjumptargetjmp:\\ popfq\\ pop rcx\\ j\textless{}cond\textgreater jumptarget\\ call faulthandler\\ fallthrough: ...\\ jumptarget: ...\end{tabular} \\ \hline
\end{tabular}
}
\label{tab:jmp}
\end{table}

==> sections/long/mov_table.tex <==
\begin{table}[h]
\caption{Local protections for {\tt mov} operation}
\centering
\begin{tabular}{lll}
\hline
\multicolumn{1}{c}{\textbf{original}}                                         & \multicolumn{1}{c}{\textbf{protected 1}}                                                             & \multicolumn{1}{c}{\textbf{protected 2}}                                                                                                \\ \hline
\begin{tabular}[c]{@{}l@{}}mov rax, {[}rbx+4{]}\\ happyflow: ...\end{tabular} & \begin{tabular}[c]{@{}l@{}}mov rax, {[}rbx+4{]}\\ mov rax, {[}rbx+4{]}\\ happyflow: ...\end{tabular} & \begin{tabular}[c]{@{}l@{}}mov rax, {[}rbx+4{]}\\ cmp rax, {[}rbx+4{]}\\ je happyflow\\ call faulthandler\\ happyflow: ...\end{tabular} \\ \hline
\end{tabular}
\label{tab:mov}
\end{table}
